Secure and Lightweight Strong PUF Challenge Obfuscation with Keyed Non-linear FSR

We propose a secure and lightweight key based challenge obfuscation for strong PUFs. Our architecture is designed to be resilient against learning attacks. Our obfuscation mechanism uses non-linear feedback shift registers (NLFSRs). Responses are directly provided to the user, without error correction or extra post-processing steps. We also discuss the cost of protecting our architecture against power analysis attacks with clock randomization, and Boolean masking. Security against learning attacks is assessed using avalanche criterion, and deep-neural network attacks. We designed a testchip in 65 nm CMOS. When compared to the baseline arbiter PUF implementation, the cost increase of our proposed architecture is 1.27x, and 2.2x when using clock randomization, and Boolean masking, respectively.

==> bios.tex <==
\vspace{-0.4in}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/khstangh}}]{Kleber Stangherlin}
Kleber received his B.Sc. in Electrical Engineering at PUCRS in Brazil. He obtained his M.Sc. in Microelectronics at UFRGS, also in Brazil. He has more than 6 years of industry experience designing security focused integrated circuits. He had key contributions to the cryptographic cores and countermeasures used in the first EAL 4+ certified chip designed in the southern hemisphere. Currently, Kleber is pursuing a PhD at University of Waterloo in Canada, where he conducts research in hardware security.
\end{IEEEbiography}

\vfill
\newpage

\vspace{-0.4in}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/zhwu}}]{Zhuanhao Wu}
Zhuanhao Wu (S'19) received the B.S. degree in computer science and technology from Nankai University, Tianjin, China in 2017, and the MASc degree in electrical and computer engineering from University of Waterloo, Ontario, Canada, in 2019, where he is currently pursuing the Ph.D. degree with the department of Electrical and Computer Engineering. His current research interests include hardware security, machine learning, and computer architecture.
\end{IEEEbiography}

\vspace{-0.4in}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/hiren}}]{Hiren Patel}
Hiren Patel is a Professor in the Department of Electrical and Computer Engineering at the University of Waterloo. Prior to the University of Waterloo, Hiren was a postdoctoral fellow at the University of California, Berkeley working in the Ptolemy group with Edward A. Lee. His research is in the design, analysis, and implementation of computer hardware and software. Currently, his research areas of interest are in real-time embedded systems, computer architecture, hardware architectures for machine learning and artificial intelligence, and security.
\end{IEEEbiography}


\vspace{-0.4in}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/msachdev}}]{Manoj Sachdev}
Manoj Sachdev is a Professor in the Department of Electrical and Computer Engineering at the University of Waterloo. He has contributed to over 225 conference and journal publications, and has written 5 books. He also holds more than 30 granted US patents. Along with his students and colleagues, he has received several international research awards. He is a Fellow of the Institute of Electrical and Electronics Engineers (IEEE), and Fellow of the Engineering Institute of Canada. Professor Sachdev serves on the editorial board of the Journal of Electronic Testing: Theory and Applications. He is also a member of program committee of IEEE Design and Test in Europe conference.
\end{IEEEbiography}

\vfill
